Security of Patched DNS

In spite of the availability of DNSSEC, which protects against cache poisoning even by MitM attackers, many caching DNS resolvers still rely for their security against poisoning on merely validating that DNS responses contain some 'unpredictable' values, copied from the re- quest. These values include the 16 bit identifier field, and other fields, randomised and validated by different 'patches' to DNS. We investigate the prominent patches, and show how attackers can circumvent all of them, namely: - We show how attackers can circumvent source port randomisation, in the (common) case where the resolver connects to the Internet via different NAT devices. - We show how attackers can circumvent IP address randomisation, using some (standard-conforming) resolvers. - We show how attackers can circumvent query randomisation, including both randomisation by prepending a random nonce and case randomisation (0x20 encoding). We present countermeasures preventing our attacks; however, we believe that our attacks provide additional motivation for adoption of DNSSEC (or other MitM-secure defenses).

==> cc.tex <==
\section{Conclusions}
Currently, most DNS resolvers defend against poisoning by validating that each response contains `unpredictable' identifiers sent in the DNS query, such as the (16 bit) query ID. Such mechanisms are clearly insufficient to prevent poisoning by MitM attackers. A secure standard alternative exists: DNSSEC, which uses cryptography to achieve verifiable security. Indeed, DNSSEC deployment is progressing - but, quite slowly. Why so slowly? One reason are significant interoperability and performance concerns; another reason may be the existence of several `patches', adding more `unpredictable' identifiers. Such `patches' are trivial to deploy and involve no or negligible overhead, hence, administrators may prefer to deploy them instead of deploying DNSSEC. \\
\indent We study all major proposed `patches', and find vulnerabilities in all of them.  
Our `trap' and `predict' attacks show that source ports may be disclosed or impacted by network devices such as NAT gateways. We show that the attacker can also nullify IP address randomisation of standard-conforming resolvers such as Unbound, forcing the resolver to query a specific name server. We also describe simple techniques to circumvent the DNS query randomisation via a random prefix and 0x20 encoding. We validated our attacks against popular NAT devices and standard DNS resolver software.
Our derandomisation attacks are deployed `sequentially' in phases, removing the randomisation of each identifier independently, and eventually strip the DNS request of the entropy offered by those `unpredictability' fields, exposing the caching DNS resolvers to efficient poisoning attacks by off-path spoofing adversaries. 

We show simple and effective countermeasures to our attacks. However, while using such `patched patches' is tempting and easy, we believe that our work shows the importance of basing security on solid, strong foundations, as provided by DNSSEC, i.e., cryptographic protocols analysed to ensure security even against MitM attackers. 

==> ctrDNSpoison.tex <==
\subsection{Improved Port Allocation Mechanism} \label{CC:S} \label{sc:short}
Official recommendations, \cite{rfc4748}, for NAT behaviour do not specify the instructions for the implementation of port allocation mechanism, as a result the developers and designers of NAT devices follow different approaches which may seem secure.
Based on our findings we identify two design factors in ports allocation mechanism of the NAT: (1) the process via which the ports are selected (i.e., random, preserving, sequential); (2) the mapping table which maintains the allocated ports.\\
{\sc Randomise Ports Selection.} Use port randomisation, but either with separate, random external port for each internal port, or at least with pseudo-random (but not sequential) increments between external port numbers\footnote{A pseudo-random permutation will provide as efficient data structure and lookup, as when using sequential allocation.}. Random ports assignment prevents the `predict' attacks.\\
{\sc Restricted Mapping Table.} 
The mapping table of allocated ports, maintained by the NAT, should be smaller than the pool of all the ports\footnote{This approach was supported only by the Checkpoint NAT which allowed it to evade our trap attacks.}, e.g., half or less of the total of number of ports; a smaller mapping table prevents the attacker from trapping the port. For each arriving packet NAT should randomly select and assign a port from the pool of ports. Each time an entry is removed from the table when the external port is freed, e.g., the entry is refreshed after a timeout, NAT should select a new random port from the pool of ports.

==> introduction.tex <==
\section{Introduction}\label{intro}
Correct and efficient operation of the Domain Name System (DNS) is essential for the operation of the Internet. 
However, there is a long history of vulnerabilities and exploits related to DNS, mostly focusing on {\em DNS poisoning}. In a poisoning attempt the attacker causes recursive DNS servers (resolvers) to cache an incorrect, fake DNS record, e.g., mapping \vicbank\ to an IP address controlled by the attacker. DNS poisoning can facilitate many other attacks, such as injection of malware, phishing, website hijacking/defacing and denial of service.

The main technique for DNS poisoning is by sending forged responses to DNS requests which were sent by resolvers; to foil this, resolvers validate responses using different mechanisms. Currently, most resolvers rely only on non-cryptographic validation, mainly, validating that the response echoes some unpredictable (random) values sent with the request, such as in the DNS ID field, the client  port, or within the resource (domain) name; e.g., see RFC 5452 \cite{rfc5452}.
Obviously, such mechanisms are insecure against a Man-in-the-Middle (MitM) attacker, who can read the randomness from the request and send a fake response with the valid identifiers. 

Furthermore, even a weaker - and more common - {\em off-path, spoofing attackers}, may be able to send valid DNS responses and cause DNS poisoning, when the validated values are predictable or limited. For example,  some DNS implementations use predictable identifiers (sequential, or using a weak pseudorandom generator); e.g., in~\cite{Klein07:Bind9Poisoning}, Klein shows how to predict the identifier for the then-current version of Bind 9, a widely-used DNS server, and how this can be exploited for highly-efficient DNS poisoning by a spoofing attacker. Indeed, as pointed out already in 1995 by Vixie \cite{Vixie95}, the identifier field alone is simply too short (16 bits) to provide sufficient defense against a determined spoofing attacker, who can foil it by sending many (but not too many) fake responses.

To improve DNS security, the IETF published DNSSEC \cite{rfc4033,rfc4034,rfc4035}, an extension to DNS, using cryptography (signatures and hashing) to ensure security (even) against MitM attackers. However, in spite of the publication of DNSSEC already in 1997 \cite{rfc2065}, and the wide awareness to its existence, deployment is still limited - e.g., less than 2\% as reported in \cite{dnssec-stat} for April, 2012. There are also many caching DNS resolvers that still do not support, or do not perform validation of, DNSSEC~\cite{olafur:nat:res}; we discuss the deployment status of DNSSEC in Appendix~\ref{sc:dnssec}. Furthermore, due to implementation errors DNSSEC protection may fail, even when both the resolver and zone deploy it: validation of signatures of important top level domains, e.g., {\sc mil}, fails since the root does not delegate the public signature key of {\sc mil} but instead provides an incorrect indication that {\sc mil} does not support DNSSEC. This results in resolvers falling back to a non-validating mode.

Indeed the deployment of DNSSEC is progressing slowly, due to challenges (see \cite{dns:derandom}), and possibly due to the recent improvements (`patches') to non-cryptographic defenses, 
causing `if it ain't broke, don\'t fix it' response. These patches are mainly by deploying new sources of `unpredictability' in DNS requests and responses, such as use of random source ports \cite{Kaminsky08,VU800113}, random DNS server selection~\cite{rfc5452} and random capitalisation of the domain name \cite{DagonAVJL08}.

This manuscript focuses on relying on such non-cryptographic `patches' to defend against DNS poisoning. This has two goals: to help improve these patches, since evidently they will remain widely used for years; and to further motivate adoption of more secure solutions such as DNSSEC, by pointing out weaknesses in the patches. While these specific weaknesses can be fixed (and we show how - often, easily), their existence should motivate the adoption of better security measures such as DNSSEC, providing security against MitM attacker and allowing for better validation of security, e.g., see \cite{bau2010security}.

\subsection{Patching Caching DNS Resolvers Against Poisoning}
Many researchers have identified vulnerabilities in the approach of relying on an `unpredictability' of some fields in a DNS request and proposed patches; we next review some of the main results. 
Bernstein, \cite{Bernstein:DNS}, suggested to improve DNS's defense against spoofed responses by sending the request from a {\em random port}, which can add a significant amount of entropy\footnote{The exact amount of entropy added depends on the number of available ports, which may be below $2^{16}$.}.
To prevent {\em birthday attack}, where attacker causes resolver to issue multiple queries for same domain in order to increase the probability of a match with one of multiple fake responses, Bernstein \cite{Bernstein:DNS} and others suggest to limit the maximal number of concurrent requests for the same resource record (to one or to some small number); this technique is usually referred to as the {\em birthday protection}. 


Many implementations did not implement these suggestions till the recent Kaminsky attack, \cite{Kaminsky08,VU800113}, which introduced two critical improvements, allowing devastating attacks on many Internet applications. 
The first improvement was to control the time at which the resolver sends queries (to which the attacker wishes to respond), by sending to the resolver queries for a non-existing host name, e.g., with a random or sequential prefix of the domain name.
The second improvement was to add, in the spoofed responses sent to the resolver, a type {\sf NS} DNS record (specifying a new name for the domain name server) and/or a type {\sf A} `glue' DNS record (specifying the IP address of that domain's name server). These records poison the resolver's entries for the victim name server. Hence, if the attack succeeds once (for one record), the adversary controls the entire name space of the victim. 

As a result of Kaminsky's attack, it became obvious that changes were needed to prevent DNS poisoning. 
Indeed, major DNS resolvers were quickly patched. 
The most basic patches were known measures - source port randomisation and birthday protection (see above). 

These and other additional patches were summarised in RFC 5452~\cite{rfc5452}, including the use of random (valid) IP addresses for the name server. 
Additional patches, implemented by some resolvers, are to randomise 
DNS queries by randomly `case toggling' the domain name (0x20 encoding \cite{DagonAVJL08}), or by adding a random prefix to the domain name \cite{DBLP:conf/dsn/PerdisciALL09}. 
It is tempting to interpret the analysis in \cite{DagonAVJL08,DagonADLLL09,rfc5452,DBLP:conf/dsn/PerdisciALL09} as indication that the `patches' may suffice to make poisoning impractical, reducing the motivation for deployment of more systematic improvements. However, we caution against this conclusion. 
This work shows that in common scenarios, attackers can often circumvent some or all of the `patches', making it still feasible to poison resolvers that rely on validation of `unpredictable' values copied from requests to responses (rather than relying on cryptographic security, as in DNSSEC).

Some concerns with `patches' were presented in earlier works. In particular, the most widely and easily deployed `patch' is clearly source port randomisation. 
However, security experts, e.g., \cite{Cross08,VU800113}, noted that DNS resolvers located behind firewall/NAT devices, that use sequential assignment of external ports, were still vulnerable to the poisoning attack. On the other hand, it was widely believed that `port-randomising' NAT devices, that sufficiently randomise the external ports, could retain or even improve the defense against DNS cache poisoning, e.g., see \cite{VU800113}. In addition, it was believed that `port-preserving' NAT devices, that leave the source port intact (if it were not already allocated to another host), can be safely used with port-randomising resolvers, e.g., see \cite{Wiki10}. Our results show otherwise, i.e., some of our attacks show how to circumvent port randomisation, in the resolver-behind-NAT scenario, even for port-randomising and port-preserving NATs. 

Note that the resolver-behind-NAT scenario is common \cite{FordSK05,rfc3489}. A recent study, \cite{olafur:nat:res}, of DNSSEC deployment by recursive resolvers observed that a large number of recursive DNS resolvers is located behind NAT devices, and often many resolvers are even behind the same NAT device. Furthermore, \cite{maier2011nat} found that $90\%$ out of 20,000 DSL lines (from a major European ISP) were located behind a NAT device.

\subsection{Attacker Model}\label{sc:atk}
In our attacks, we assume an off-path, spoofing adversary connected to the Internet and a non-spoofing (user-mode) compromised host (zombie) on the local network; such zombies exist in many networks, e.g., see~\cite{bot:survey}; the attacker model is depicted in Figure~\ref{DNSpunchingNet:F}, in the Appendix. The zombie can open user mode sockets and can send arbitrary (non-spoofed) packets, ~\cite{dns:survey3}. 
Alternately, the attacker can poison a DNS resolver which provides open recursion services.

Note that, in many scenarios, attackers do not even need to infiltrate malware to be able to control a host inside a local area network, e.g., attackers can obtain legitimate temporary access to organisational or other networks, or can connect to wireless networks as a legitimate client.

\subsection{Our Contributions}
The security of patched DNS resolvers relies on the randomness provided by the validation fields. We show that it is possible to reduce and often to nullify the randomness, thereby exposing the resolvers to Kaminsky style poisoning attacks. Our attacks apply to all widely-deployed `patches':\\
{\sc source-port randomisation.} We expose vulnerabilities in common source ports allocation algorithms, used by popular NAT devices; see Section~\ref{sc:ttp}. 
The vulnerabilities allow to predict the source port allocated to queries of the resolver. 
We tested our attacks in a lab setting against several NAT devices, see Table~\ref{T:nat}. The type of the NAT that the resolver resides behind is important in deciding which attack to launch. \\
{\sc DNS server IP randomisation.} We present techniques to predict (or force) the IP address of the name server to which the resolver will send its DNS request, see Section~\ref{sc:ip}. Our techniques rely on fragmented DNS responses.\\
{\sc domain name randomisation.} We further show that randomisation of DNS queries via 0x20 or by prepending a random string is not always effective and does not introduce protection against poisoning attacks; see Section~\ref{sc:0x20}.\\
In addition to presenting the vulnerabilities, we also propose countermeasures; however, our most important contribution may be in motivating the adoption of systematic, secure defenses against poisoning, such as DNSSEC. 




==> x20Plus.tex <==
\section{DNS Query (de)Randomisation}
\label{sc:0x20} %\label{WSEC:SS}
In this section we describe two prominent defenses, `case toggling' and random prefix, which are known to add significant extra entropy to DNS requests and show simple ways to circumvent them.\\
\indent {\sc `cASe toGgLiNg'.} Dagon et al. \cite{DagonAVJL08} present {\em 0x20 encoding} for prevention of DNS poisoning. The technique is to randomly toggle the case of letters of which the domain name consists, and validate them in response. 
If the domain name $d$ contains $l(d)$ alphabetic characters, this increases the space of identifiers by a factor of $X(d)=2^{l(d)}$. For example, a typical domain name, e.g., www.google.com, would increase the attacker's search space by a factor of $X(\textsc{www.google.com})=2^{12}$. Of course, the factor $X$ depends on the number of alphabetic characters in the domain name, e.g., $X(\textsc{a9.com})=2^4$. 
However, we believe that the distribution of domain queries with sufficient 0x20 characters, as reported by  Dagon et al., is not indicative of the number of characters in queries that attackers will try to poison, and hence the impact of 0x20 encoding can be easily circumvented.
In fact, in Kaminsky-style attacks, the query is intentionally for a non-existing domain name chosen by the attacker,
e.g., the Top Level Domains (TLDs) such as {\sc .com} and {\sc .uk}; indeed the attackers prefer to poison a response to {\sc com} rather than to {\sc www.google.com}. Poisoning {\sc com} allows the attacker a control over all subdomains of {\sc com} (including {\sc www.google.com}). 
Therefore, although 0x20 encoding provides significant extra entropy for long domain names, 
 the attacker will choose to poison `high value' TLDs, thereby circumventing the protection of 0x20.\\
 \indent {\sc Random Prefix.} Prepending a random prefix to a DNS query\footnote{A random prefix is a variation of the defense proposed in \cite{DBLP:conf/dsn/PerdisciALL09}.} can ensure that a sufficiently large DNS query is sent, allowing to apply the 0x20 encoding on more letters and also making it more difficult for the attacker to guess the query (and the case of each letter). \\
\indent The DNS query is composed of subdomains, at most 63 bytes each, separated by dots and at the right end the query ends with a top level domain, e.g., {\sc subdomain.subdomain.subdomain.subdomain.TLD}. The total number of characters cannot exceed 255 bytes. So, prepending a random string \$1 to query {\sc abc.tld}, results in {\sc \$1.abc.tld} and increases the query by the size of \$1.\\
\indent But as we show this protection can also be foiled by the attacker. 
The attacker that wishes to poison an entry for some top level domain, e.g., {\sc com}, can issue a maximal size DNS query, i.e., 255 bytes, consisting of numbers, that will not allow prepending any more characters: {\sc 1-36.1-36.1-36.1-33.com} (the `1-36' denotes a string containing all numbers between 1 and 36). As a result, the attacker circumvents the 0x20 protection (which does not apply to numbers) and further avoids the addition of a random prefix to DNS request (since the query is already of maximal size). We tested the reduction of query randomisation (and foiling of 0x20) against Google Public DNS, \cite{google:dns}, which supports both defenses, i.e., 0x20 and random prefix. A slight variation of this attack, see \cite{dns:derandom}, also foils protection offered by WSEC DNS~\cite{DBLP:conf/dsn/PerdisciALL09}.\\
\indent Such long queries to top level domains should be restricted or should receive a special treatment, yet we are not aware of appropriate recommendations in the relevant documentation.
